Efficient high-quality motion planning by fast all-pairs r-nearest-neighbors

Sampling-based motion-planning algorithms typically rely on nearest-neighbor (NN) queries when constructing a roadmap. Recent results suggest that in various settings NN queries may be the computational bottleneck of such algorithms. Moreover, in several asymptotically-optimal algorithms these NN queries are of a specific form: Given a set of points and a radius r report all pairs of points whose distance is at most r. This calls for an application-specific NN data structure tailored to efficiently answering this type of queries. Randomly transformed grids (RTG) were recently proposed by Aiger et al. as a tool to answer such queries and have been shown to outperform common implementations of NN data structures in this context. In this work we employ RTG for sampling-based motion-planning algorithms and describe an efficient implementation of the approach. We show that for motion-planning, RTG allow for faster convergence to high-quality solutions when compared with existing NN data structures. Additionally, RTG enable significantly shorter construction times for batched-PRM variants; specifically, we demonstrate a speedup by a factor of two to three for some scenarios.

==> alg.tex <==
\section{Asymptotically near-optimal motion-planning}
\label{sec:alg}
Clearly the asymptotic optimality of the RRT* and RRG algorithms come at the cost of the additional $k_{RRG}\log(|V|)-1$ calls to the local planner at each stage (and some additional overhead).
If we are not concerned with \emph{asymptotically optimal} solutions, we do not have to consider all of the $k_{RRG} \log(|V|)$ neighbors when a node is added. 
Our idea is to initially only assess the quality of each edge.
We use the quality of the edge to decide if to 
discard it, 
use it \emph{without} checking if it is collision-free or 
use it after validating that it is indeed collision-free.
%Certain edges can be discarded without checking if they are collision-free as they will not improve the quality of paths maintained by the algorithm.  Other edges can be assumed lazily to be collision-free and only if needed will the local planner be called. 
%Finally, the local planner will be called for the remaining edges.
Thus, many calls to the local planner can be avoided, though we still need to estimate the quality of many edges. 
Our approach is viable in cases where such an assessment can be carried out efficiently, namely more efficient than deciding if an edge is collision-free.
This condition holds naturally when the quality measure is path length.


\subsection{Notation}
Let $\Sigma$ be the set of all feasible paths,
$c: \Sigma \rightarrow \R^+$ a cost function and
$c^*$ denote the \emph{optimal cost}.
Namely, $c^* = \min_{\sigma \in \Sigma} \set{c(\sigma)}$.
In this paper we only consider \emph{path length} as the cost function.
Let $\sigma_{\text{ALG}}(n)$ be the path produced by 
\textVersion{an}{a sampling-based}
 algorithm ALG using $n$ free samples.
\textVersion{It}{An algorithm ALG} is \emph{asymptotically optimal} if 
$\lim_{n \rightarrow \infty} c(\sigma_{\text{ALG}}(n)) = c^*$
with probability one and 
\emph{asymptotically $(1+\varepsilon)$-optimal} if 
$\lim_{n \rightarrow \infty} c(\sigma_{\text{ALG}}(n)) \leq (1+\varepsilon) \cdot c^*$
with probability one.
We refer to an algorithm that computes an asymptotically $(1+\varepsilon)$-optimal path as \emph{asymptotically near-optimal} and  to $(1+\varepsilon)$ as the \emph{approximation~factor}.
%We refer to an asymptotically $(1+\varepsilon)$-optimal algorithm as \emph{asymptotically near-optimal} and  to $(1+\varepsilon)$ as the \emph{approximation~factor}.

Let \texttt{order}$_\calG(X,x)$ be a procedure which returns the elements of $X$ ordered according to the cost to reach $x$ from $x_{init}$ through an element $x'$ of $X$.
Namely, after ordering, $x_1\in X$ is before $x_2 \in X$ if 
$\texttt{cost}_{\calG}(x_1) + \texttt{cost}(x_1, x) 
	\leq 
 \texttt{cost}_{\calG}(x_2) + \texttt{cost}(x_2, x)$.
The importance of this ordering will be discussed in the next~subsection.

\subsection{\eRRT}
We propose a modification to the RRT* algorithm by maintaining two roadmaps $\Tlb, \Tub$ simultaneously.
Each roadmap is a tree rooted at $x_{init}$ and consist of the same set of vertices but differ in their edge set\footnote{The subscript of \Tlb is an abbreviation for lower bound and the subscript of \Tub is an abbreviation for approximation.}. 


Let $\calG_{RRG}$ be the roadmap constructed by RRG if run on the same sequence of samples used for \eRRT.
Now, $\Tlb, \Tub$  maintain the following invariants throughout the algorithm:\\
\textVersion{\vspace{-5mm}}{}
\begin{framed}
\textbf{Bounded approximation invariant} - 
For every node $x \in \Tub, \Tlb$,
$
	\texttt{cost}_{\Tub}(x) 
			\leq 
	(1+\varepsilon) \cdot \texttt{cost}_{\Tlb}(x).
$
\end{framed}
\textVersion{\vspace{-2mm}}{}
and
\textVersion{\vspace{-2mm}}{}
\begin{framed}
\textbf{Lower bound invariant} - 
For every node $x \in \Tub, \Tlb$,
$
	\texttt{cost}_{\Tlb}(x) \leq \texttt{cost}_{\calG_{RRG}}(x).
$
\end{framed}
The lower bound invariant is maintained by constructing $\Tlb$ as a subgraph of $\calG_{RRG}$, with possibly some additional edges that are not collision-free, containing only the best route to each node.
Notice that the cost of an edge, regardless of whether it is collision-free or not, is the length of the segment connecting its end configurations.
 
The main body of the algorithm (see Algorithm~\ref{alg_RRT}) follows the structure of the RRT, RRT* and RRG algorithms with respect to adding a new milestone (lines 3-7) but differs in the connections added.
If a path between the new node $x_{new}$ and its nearest neighbor $x_{nearest}$ is indeed collision-free, it is added to both trees with an  edge from $x_{nearest}$ to $x_{new}$ (lines~8-10).
This is demonstrated in Figure~\ref{fig:adding_node}.

Similar to RRT*, \eRRT locates the set $X_{near}$ of $k_{RRG}\log(|V|)$ nearest neighbors of $x_{new}$ (line~11).
Then, it uses a rewiring procure 
\textVersion{\texttt{rewire}}{\texttt{rewire\_\eRRT}}
(Algorithm~\ref{alg_update}) to assess 
\textbf{(i)}~which node $x_{near} \in X_{near}$ should be the parent of $x_{new}$ in each tree (lines~13-14)
 and 
\textbf{(ii)}~if $x_{new}$ may improve the cost to reach any node $x_{near} \in X_{near}$ in each tree  (lines~15-16).
If so, the roadmaps are updated.
In contrast to RRT* where rewiring is \emph{always} performed, \eRRT only performs rewiring that is necessary to maintain the two invariants.

Given two nodes $x_{potential\_parent}$, $x_{child}$, 
the subroutine \textVersion{\texttt{rewire}}{\texttt{rewire\_\eRRT}} (Algorithm~\ref{alg_update}) checks if an edge should be added between $x_{potential\_parent}$ and $x_{child}$.
If so, the newly introduced edge replaces the existing edge between the parent of $x_{child}$ and $x_{child}$ (namely a rewiring occurs).
Initially the cost $potential\_cost_{lb}$ to reach $x_{child}$ in $\Tlb$ using $x_{potential\_parent}$ as the parent of $x_{child}$ is computed (lines~1-2).
The cost of the existing path to $x_{child}$ in $\Tlb$ is either 
\textbf{(i)}~smaller than $potential\_cost_{lb}$,
\textbf{(ii)}~larger than $potential\_cost_{lb}$ and  rewiring would violate  the bounded approximation invariant or
\textbf{(iii)}~larger than $potential\_cost_{lb}$ but rewiring would not violate the bounded approximation invariant.

Each of the above cases is handled by Algorithm~\ref{alg_update}:
If the cost of the existing path to $x_{child}$ in $\Tlb$ is lower than  $potential\_cost_{lb}$ (case (i)), then no action is taken (lines 3-4 and Figure~\ref{fig:line3}).
If not, then a potentially lower-cost path may exist (recall that the edge between $x_{potential\_parent}$ and $x_{child}$ may not be collision-free).
If the bounded approximation invariant is violated (case~(ii), line 5 and Figure~\ref{fig:line5}), then one must explicitly check if the connection is collision-free (line 6). 
If this is indeed the case then both $\Tlb$ and $\Tub$ are rewired.
If the cost does not violate the bounded approximation invariant (case~(iii), line~9 and Figure~\ref{fig:line9}) then% 
\textVersion{}{ we assume lazily that the connection is collision-free and} only $\Tlb$ is rewired (line~10 and Figure~\ref{fig:line10}).

\begin{algorithm}[t,b]
\caption{\eRRT ($x_{init}, \varepsilon$ )}
\label{alg_RRT}
\begin{algorithmic}[1]
 \STATE $\Tlb.V \leftarrow \set{x_{init}}$
 				\hspace{3mm}
 				$\Tub.V \leftarrow \set{x_{init}}$
 \WHILE {build\_tree()}
 	\textVersion{\vspace{2mm}}{\vspace{3mm}}

 	\STATE $x_{rand} \leftarrow \texttt{sample\_free()}$
 	\STATE $x_{nearest} \leftarrow
 											\texttt{nearest\_neighbor}(	x_{rand}, \Tlb.V)$
 	\STATE $x_{new} \leftarrow
 											\texttt{steer}(	x_{nearest}, x_{rand})$
 	\textVersion{\vspace{2mm}}{\vspace{3mm}}
 	
 	\IF {(!\texttt{collision\_free}($x_{nearest}, x_{new}$))}
 		\STATE CONTINUE
	\ENDIF
 	\textVersion{\vspace{2mm}}{\vspace{3mm}}
 	
 	\STATE	$\Tlb.V \leftarrow \Tlb.V \cup \set{x_{new}}$
 					\hspace{3mm}
 					$\Tub.V \leftarrow \Tub.V \cup \set{x_{new}}$
 	\STATE	$\Tlb.\texttt{parent}(x_{new}) \leftarrow x_{nearest}$
 	\STATE	$\Tub.\texttt{parent}(x_{new}) \leftarrow x_{nearest}$
  \vspace{3mm}

  \STATE $X_{near} \leftarrow \texttt{nearest\_neighbors}(	x_{new},$\\ 
  			\hspace{35mm}
  			$\Tlb.V , k_{RRG} \log(|\Tlb.V |))$

  
  \STATE $X_{ordered} \leftarrow
        \texttt{order}_{\Tlb}(	X_{near}, x_{new})$

	\textVersion{\vspace{2mm}}{\vspace{3mm}}
  
	\FORALL {$(x_{near}, X_{ordered})$}
  	\STATE  \textVersion{\texttt{rewire}}{\texttt{rewire\_\eRRT}}
  					($x_{near}, x_{new}$ )
%  	\hspace{7 mm}
%  	//UPDATE INCOMING PATHS TO $x_{new}$ 
  \ENDFOR

	\textVersion{\vspace{2mm}}{\vspace{3mm}}
  
	\FORALL {$(x_{near}, X_{near})$}
  	\STATE  \textVersion{\texttt{rewire}}{\texttt{rewire\_\eRRT}}
  					($x_{new}, x_{near}$ )
%    \hspace{7 mm}
%    //REWIRE OUTGOING PATHS FROM $x_{new}$ 	        
  \ENDFOR
 \ENDWHILE
 	
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[t,b]
\textVersion
{\caption {\texttt{rewire}($x_{potential\_parent}, x_{child}$)}}
{\caption{\texttt{rewire\_\eRRT}($x_{potential\_parent}, x_{child}$)}}
\label{alg_update}
\begin{algorithmic}[1]
	\STATE	$c \leftarrow$ \texttt{cost}($x_{potential\_parent}, x_{child}$)
  \STATE	$potential\_cost_{lb} \leftarrow 
  						cost_{\Tlb}(x_{potential\_parent}) + c$
	\textVersion{\vspace{2mm}}{\vspace{3mm}}
  
  \IF {	($\texttt{cost}_{\Tlb}(x_{child}) \leq potential\_cost_{lb} )$}
  	\RETURN
  \ENDIF
  \textVersion{\vspace{2mm}}{\vspace{3mm}}
    
  \IF {	$	(\texttt{cost}_{\Tub}(x_{child})  > (1+\varepsilon) \cdot 
  				potential\_cost_{lb} )$}
	  \IF {(\texttt{collision\_free}($x_{potential\_parent}, x_{child}$))}
        
	    \STATE	$\Tlb.\texttt{parent}(x_{child}) \leftarrow 
    						x_{potential\_parent}$
	    \STATE	$\Tub.\texttt{parent}(x_{child}) \leftarrow 
    						x_{potential\_parent}$
    \ENDIF
	
  \ELSE
    \STATE	$\Tlb.\texttt{parent}(x_{child}) \leftarrow 
    						x_{potential\_parent}$
 	\ENDIF

\end{algorithmic}
\end{algorithm}						


Now we can explain the advantage in ordering the nodes (Algorithm~\ref{alg_RRT}, line 12).
The set $X_{near}$ will be traversed from the node that may yield the lowest bound to reach $x_{new}$ to the node that will yield the highest lower bound (Algorithm~\ref{alg_RRT}, lines 13-14).
After the first rewiring, either with or without a call to the collision detector (Algorithm~\ref{alg_update} lines 7,8 and line~10, respectively), no subsequent node can improve the cost to reach $x_{new}$.
Indeed, after such rewiring, for each subsequent node, Algorithm~\ref{alg_update} will not contain any (computationally demanding) calls to the collision detector.
We note that this ordering is used in practice to speed up~RRT*. 

\subsection{Analysis}
\textVersion{We}{In this section we	} show that Algorithm~\ref{alg_RRT} maintains the lower bound invariant (Corollary~\ref{cor_lb}) and 
that after every iteration% 
\textVersion{}{ of the algorithm} %
the bounded approximation invariant is maintained (Lemma~\ref{lem_invariant}).
%aaaaaaaaaaaaaaaaaaaaa

We note the following (straightforward, yet helpful) observations comparing \eRRT, RRG and RRT* when run on the same set of random samples:
\begin{obs}
\label{obs:1}
A node is added to $\Tlb$ and to $\Tub$ if and only if a node is added to $\calG_{RRG}$ 
\textVersion
{%ICRA version - no reference to RRG algorithm
(Algorithm~\ref{alg_RRT}, lines 3-8). 
}
{%ARXIV version - refer to RRG algorithm
(see Algorithm~\ref{alg_RRG} and Algorithm~\ref{alg_RRT}, lines 3-8). 
}
\end{obs}
\begin{obs}
Both \eRRT and RRG consider the same set of $k_{RRG}\log(|V|)$ nearest neighbors of~$x_{new}$%
\textVersion
{%ICRA version - no reference to RRG algorithm
~(Algorithm~\ref{alg_RRT}, line~11).
}
{%ARXIV version - refer to RRG algorithm
~(see Algorithm~\ref{alg_RRG}, line~10 and Algorithm~\ref{alg_RRT}, line~11).
}
\end{obs}
\begin{obs}
 $\Tlb$ undergoes the same rewiring process as RRT* (see Algorithm~\ref{alg_update}, lines~7,~10) with possibly some additional edges that are not collision-free (see Algorithm~\ref{alg_update}, line~10).
\end{obs}
\begin{obs}
\label{obs:4}
Every edge of $\Tub$ is collision free~(see Algorithm~\ref{alg_RRT}, line 10 and Algorithm~\ref{alg_update}, line~8).
\end{obs}

Thus, the following corollary trivially holds:
\begin{cor}
\label{cor_lb}
	For each node $x \in \Tlb$, $\texttt{cost}_{\Tlb}(x) \leq \texttt{cost}_{\calG_{RRG}}(x)$
\end{cor}
%\begin{cor}
%\label{lem_ub}
%	$\Tub$ is a subgraph of the RRG roadmap
%\end{cor}

Using Observations~\ref{obs:1} through~\ref{obs:4} and Corollary~\ref{cor_lb}, 
%we obtain:
\begin{lem}
\label{lem_invariant}
	After every iteration of Algorithm~\ref{alg_RRT} (lines 3-16) the bounded approximation invariant is maintained.
\end{lem}

\begin{proof}
The edges of $\Tlb, \Tub$ are updated in one of the following cases:\\
\textbf{case (a):}
When adding a new milestone $x_{new}$ to the trees, it is initially connected in both trees to the same milestone $x_{nearest}$ (see Algorithm~\ref{alg_RRT}, lines 8-10).
\textVersion
{
Assume that the invariant was maintained prior to this step. Then,
\vspace{-3mm}
\begin{eqnarray}
\texttt{cost}_{\Tub}(x_{new})
		&		= 	&		
\texttt{cost}_{\Tub}(x_{nearest}) + 
 		\nonumber \\
		&			&		\texttt{cost}(x_{nearest}, x_{new})
 		\nonumber \\
		&		\leq 	&		
(1+\varepsilon) \cdot \texttt{cost}_{\Tlb}(x_{nearest}) + 
 		\nonumber \\
		&			&		\texttt{cost}(x_{nearest}, x_{new})
 		\nonumber \\
		&		\leq 	&		
(1+\varepsilon) \cdot  \texttt{cost}_{\Tlb}(x_{new}). \nonumber 
\end{eqnarray}
\vspace{-3mm}
}
{
Assume that the invariant was maintained prior to this step, namely:
\[
		\texttt{cost}_{\Tub}(x_{nearest}) 
			\leq 
	(1+\varepsilon) \cdot \texttt{cost}_{\Tlb}(x_{nearest}).
\]
Using the invariant, 
\begin{eqnarray}
\texttt{cost}_{\Tub}(x_{new})
		&		= 	&		
\texttt{cost}_{\Tub}(x_{nearest}) + 
 		\nonumber \\
		&			&		\texttt{cost}(x_{nearest}, x_{new})
 		\nonumber \\
		&		\leq 	&		
(1+\varepsilon) \cdot \texttt{cost}_{\Tlb}(x_{nearest}) + 
 		\nonumber \\
		&			&		\texttt{cost}(x_{nearest}, x_{new})
 		\nonumber \\
		&		\leq 	&		
(1+\varepsilon) \cdot  \texttt{cost}_{\Tlb}(x_{new}). \nonumber 
\end{eqnarray}
}

\textbf{case (b):}
Additional rewiring may occur in Algorithm~\ref{alg_update}, line 5.
%This occurs when 
%$	(\texttt{cost}_{\Tub}(x_{child})  > (1+\varepsilon) \cdot 
%  				potential\_cost_{lb} )$.
In this case both trees update the incoming edge of $x_{child}$ to be $x_{potential\_parent}$. 
Assuming that the invariant was maintained prior to this step then it is maintained after this update (see case (a), only that now we use $x_{potential\_parent}$ instead of $x_{nearest}$).

\textbf{case (c):}
Finally rewiring may also occur in Algorithm~\ref{alg_update}, line 10.
This occurs when 
$	(\texttt{cost}_{\Tub}(x_{child})  \leq (1+\varepsilon) \cdot 
  				potential\_cost_{lb} )$. 
In this case only $\Tlb$ is updated and:
\begin{eqnarray}
 \texttt{cost}_{\Tub}(x_{child}) 
 		&		\leq 	&		
 	(1+\varepsilon) \cdot   potential\_cost_{lb} 
 		\nonumber \\
		&		= 	&		
 (1+\varepsilon) \cdot  \texttt{cost}_{\Tlb}(x_{child}).
		\nonumber 
\end{eqnarray}
\end{proof}

From 
Corollary~\ref{cor_lb},
Lemma~\ref{lem_invariant} and
using the asymptotic optimality of RRG:
\begin{thm}
 	\eRRT is asymptotically near-optimal with an approximation factor of $(1+\varepsilon)$. 
\end{thm}
\textVersion
{
}
{
\noindent
Namely the cost of the path computed by \eRRT converges to a cost lower than $(1+\varepsilon)$ times the cost of the optimal path almost surely.	
}


%\vspace{-3mm}
\subsection{Discussion}
%\eRRT allows for an interpolation between the fast RRT algorithm and the asymptotically optimal RRT* algorithm. 
Let ${\rm T}_{ALG}^{\omega}$ denote the time needed for an algorithm $ALG$ to find a feasible solution on a set of random samples $\omega$. 
Clearly, ${\rm T}_{\rm RRT}^{\omega} \leq {\rm T}_{\rm RRT^*}^{\omega}$ (as the RRT* algorithm may require more calls to the collision detector than the RRT algorithm).
Moreover for every $\varepsilon_1 \leq \varepsilon_2$ it holds that 
\[
%T_{\eRRT(\infty)}^{\omega} 
{\rm T}_{\rm RRT}^{\omega} 
	\leq 
{\rm T}_{\rm \eRRT(\varepsilon_2)}^{\omega} 
	\leq
{\rm T}_{\rm \eRRT(\varepsilon_1)}^{\omega} 
	\leq 
{\rm T}_{\rm RRT^*}^{\omega}.
%T_{\eRRT(0)}^{\omega}.
\]

Thus, given a limited amount of time, RRT* may fail to construct any solution. 
On the other hand, RRT may find a solution fast but will not improve its quality (if the goal is a single configuration).
\eRRT allows to find a feasible path quickly while 
continuing to search for a path of higher quality.

\textVersion
{
RRT and RRT* have been used in numerous applications and various implementations and heuristics have been suggested for them.
Typically, the applications rely on the efficiency of RRT or the asymptotic optimality of RRT*.

We argue that \eRRT can replace RRT and RRT* in many applications.
If the overhead of running \eRRT when compared to RRT is acceptable%
\textVersion{}
{ (which may indeed be the case as the experimental results in Section~\ref{sec:eval} suggest)}%
, then the algorithm will be able to produce \emph{high-quality} paths in different settings.
Additionally, if one is concerned with \emph{fast convergence} to a high quality solution, 
\eRRT can  replace RRT* seamlessly, trading the asymptotic optimality with a weaker near-optimality guarantee.
For a partial list of examples where \eRRT can replace RRT or RRT*, the reader is referred to~\cite{SH13-arxiv}.

Efficient implementations and heuristics typically take into account the primitive operations used by the RRT and the RRT* algorithms (such as collision detection, nearest neighbor computation, sampling procedure etc.).
Thus, techniques suggested for efficient implementations of RRT and RRT* may be applied to \eRRT with little effort as the latter relies on the same primitive operations.
Again, for a partial list of examples, the reader is referred to~\cite{SH13-arxiv}.
}
{
}



==> conclusion.tex <==
%\section{Conclusion and Future work}
\section{Future work}
\label{sec:con}
We seek to suggest natural stopping criteria for \eRRT.
Such criteria could possibly be related to the rate at which the quality is increased as additional samples are introduced.
Once such a criterion is established, one can think of the following  framework:
Run \eRRT with a large approximation factor%
\textVersion{}{ (large $\varepsilon$)}%
, once the stopping criterion has been met, decrease the approximation factor and continue running.
This may allow an even quicker convergence to find any feasible path while allowing for refinement as time permits (similar to~\cite{APD11}).

\textVersion
{Additionally, we wish to apply our framework to different quality measures.}
{An interesting question to be further studied is can our framework be applied to different quality measures.}
For certain measures, such as bottleneck clearance of a path, this is unlikely (as bounding the quality of an edge already identifies if it is collision-free). 
However, for measures such as energy consumption, the framework may be used.

%Finally, we wish to explore the behavior of our algorithm given a \emph{fixed, limited} time budget. 
%This analysis should take into account the different homotopy classes and the probability that the algorithm will find each one using a given fixed number of samples.
